Computational acceleration strategies for large-scale energy system optimization: a comparative study of GPU-accelerated and distributed-memory solvers

Energy system optimization models are increasing in scope and resolution, yielding large and challenging linear programs. For a long time, the standard way to address such problems has relied on shared-memory interior-point methods (IPM), which combine robustness and accuracy but face scalability limits as model instance size grows. Recently, two promising directions for specialized solver architectures have emerged: (i) GPU-accelerated first-order methods (FOM); and (ii) distributed-memory IPM, which can exploit block structure that arises in many energy system models. This paper presents a computational study comparing these solver classes on a diverse test set of large-scale linear programs arising from energy system analysis, including scenario-based formulations derived from stochastic programming. The results illustrate that distributed-memory IPM can leverage problem structure to deliver substantial speed-ups on specific problems with block-angular structures. GPU-accelerated FOMs demonstrate strong scalability but may yield solutions with higher relative infeasibilities, which, depending on the use case and model uncertainty, can still be acceptable. Overall, our findings indicate that recent algorithmic and hardware advances substantially broaden the computational toolbox available to the energy system optimization community. Each solver class exhibits distinct advantages: shared-memory IPMs remain a powerful tool for reliably obtaining high-accuracy solutions; distributed-memory IPMs can extend scalability to hundreds of cores for certain structured models, enabling faster time-to-solution; and GPU-based FOM can deliver fast solutions when such lower accuracy levels are appropriate. Together, they help make high-resolution, multi-scenario energy system optimization models tractable across a broader range of problem sizes and computing environments.

==> experiment_table.tex <==
\begin{longtable}{llllllll}
\hline
Instance & Solver & Thr & Method & Time & Iter & Status & Obj \\
\hline
\endfirsthead
\hline
Instance & Solver & Thr & Method & Time & Iter & Status & Obj \\
\hline
\endhead
288\_22\_8 & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 86403 & 59-61 & Time limit reached & 0 \\
288\_22\_8 & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 86403 & 60 & Time limit reached & 0 \\
672\_22\_8\_cli & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo & 86804 & 38 & Time limit reached & 0 \\
672\_22\_8\_cli & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 86406 & 38 & Time limit reached & 0 \\
672\_22\_8\_cli & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 86447 & 38 & Time limit reached & 0 \\
Adalpert & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo & 86669 & 84-90 & Time limit reached & 0 \\
Adalpert & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo & 86456 & 92 & Time limit reached & 0 \\
Adalpert & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 86410 & 92 & Time limit reached & 0 \\
DTU\_Y3FF\_S52\_T48\_C5 & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 81489 & 95 & \makecell[l]{Solve error, \\ Time limit reached} & 0 \\
DTU\_Y3FF\_S52\_T48\_C5 & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 81581 & 95 & \makecell[l]{Solve error, \\ Time limit reached} & 0 \\
ELMOD\_438\_20\_noVEnames & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo & 51 & not found & Infeasible & 0 \\
ELMOD\_438\_20\_noVEnames & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo & 50 & not found & Infeasible & 0 \\
JRC-EU-TIMES-30-12ts & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo & 20 & not found & Infeasible & 0 \\
JRC-EU-TIMES-30-12ts & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo & 18 & not found & Infeasible & 0 \\
\makecell[l]{JRC-EU-TIMES-dispatch-30- \\ 2016ts} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo & 42 & not found & Infeasible & 0 \\
\makecell[l]{JRC-EU-TIMES-dispatch-30- \\ 2016ts} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo & 41 & not found & Infeasible & 0 \\
\makecell[l]{SWITCH-China-open-model-3 \\ 2-433ts} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 8269 & 77 & Unknown & 3.418651851e+12 \\
\makecell[l]{SWITCH-China-open-model-3 \\ 2-433ts} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 7837 & 77 & Unknown & 3.418651851e+12 \\
\makecell[l]{TIMES-GEO-global-base-31- \\ 20ts} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 6752 & 213 & Unknown & 242284270.9 \\
\makecell[l]{TIMES-GEO-global-base-31- \\ 20ts} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 6290 & 213 & Unknown & 242284270.9 \\
\makecell[l]{TIMES-GEO-global-netzero- \\ 31-20ts} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 1938 & 86 & Unknown & 5.229565656e+12 \\
\makecell[l]{TIMES-GEO-global-netzero- \\ 31-20ts} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 2168 & 86 & Unknown & 5.229565656e+12 \\
TIMES-STEM-15-1h & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo & 14 & not found & Infeasible & 0 \\
TIMES-STEM-15-1h & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo & 17 & not found & Infeasible & 0 \\
\makecell[l]{YSSP\_disp\_488r\_t\_1460b\_no \\ venames} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 86407 & 8-9 & Time limit reached & 0 \\
\makecell[l]{YSSP\_disp\_488r\_t\_1460b\_no \\ venames} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 86403 & 9 & Time limit reached & 0 \\
\makecell[l]{elec\_s\_DE5\_AT10\_lv1.0\_\_Co \\ 2L0p79-120h-T-H-B-I-W\_2015} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 86409 & 70 & Time limit reached & 0 \\
\makecell[l]{elec\_s\_DE5\_AT10\_lv1.0\_\_Co \\ 2L0p79-120h-T-H-B-I-W\_2015} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 86415 & 70 & Time limit reached & 0 \\
\makecell[l]{ethos\_fine\_europe\_60tp-17 \\ 5-720ts} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 86401 & 71-75 & Time limit reached & 0 \\
\makecell[l]{ethos\_fine\_europe\_60tp-17 \\ 5-720ts} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 86401 & 70-76 & Time limit reached & 0 \\
fxe6qfja & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 86404 & 6 & Time limit reached & 0 \\
fxe6qfja & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 86404 & 6 & Time limit reached & 0 \\
genx-elec\_co2-15-168h & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 20839 & 73 & Unknown & 456466.291 \\
genx-elec\_co2-15-168h & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 19997 & 73 & Unknown & 456466.291 \\
genx-elec\_trex-15-168h & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 86402 & 89-90 & Time limit reached & 0 \\
genx-elec\_trex-15-168h & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 86402 & 88-89 & Time limit reached & 0 \\
\makecell[l]{genx-elec\_trex\_co2-15-168 \\ h} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 21451 & 73 & Unknown & 460885.4891 \\
\makecell[l]{genx-elec\_trex\_co2-15-168 \\ h} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 20039 & 73 & Unknown & 460885.4891 \\
\makecell[l]{nt2030\_2030\_CY2009\_st1\_12 \\ 0b} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo & 2485 & 136 & Unknown & 643530.2132 \\
\makecell[l]{nt2030\_2030\_CY2009\_st1\_12 \\ 0b} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo & 2587 & 136 & Unknown & 643530.2132 \\
oemofB3\_int\_125 & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 86630 & 63 & Time limit reached & 0 \\
oemofB3\_int\_125 & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 86483 & 63 & Time limit reached & 0 \\
oemofB3\_int\_250 & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 44832 & not found & Solve error & not found \\
oemofB3\_int\_250 & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 46120 & not found & Solve error & not found \\
oemofB3\_int\_37 & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 86428 & 34 & Time limit reached & 0 \\
oemofB3\_int\_37 & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 86434 & 34-35 & Time limit reached & 0 \\
\makecell[l]{spineopt-multiyear-invest \\ -eu-case-study} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 86400 & 100-101 & Time limit reached & 0 \\
\makecell[l]{spineopt-multiyear-invest \\ -eu-case-study} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 80500 & 103 & Unknown & 1.556382778e+13 \\
subCWE\_1h\_ticapin\_40b & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 113337 & 77 & Time limit reached & 0 \\
subCWE\_1h\_ticapin\_40b & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 123220 & 77 & Time limit reached & 0 \\
\makecell[l]{zen-garden-eur-PI-annual- \\ emission-limit-28-100ts} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 86401 & 85-87 & Time limit reached & 0 \\
\makecell[l]{zen-garden-eur-PI-annual- \\ emission-limit-28-100ts} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 86401 & 88-89 & Time limit reached & 0 \\
\makecell[l]{zen-garden-eur-PI-constra \\ ined-expansion-28-100ts} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 16 & hipo, IPX & 53220 & 10 & Unknown & -3.631348295e+10 \\
\makecell[l]{zen-garden-eur-PI-constra \\ ined-expansion-28-100ts} & \makecell[l]{HiGHS 1.12.0 \\  (f32c3cb02)} & 32 & hipo, IPX & 49178 & 10 & Unknown & -3.631348295e+10 \\
\hline
\caption{Overview Experiments Shared Memory IPM. \\
Hardware: Intel(R) Xeon(R) Gold 6342 CPU @ 2.80GHz. \\
Convergence Tolerance: 1e-6 for "ipm\_optimality\_tolerance"}
\end{longtable}

\begin{longtable}{llllllll}
\hline
Instance & Solver & Thr & Method & Time & Iter & Status & Obj \\
\hline
\endfirsthead
\hline
Instance & Solver & Thr & Method & Time & Iter & Status & Obj \\
\hline
\endhead
288\_22\_8 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 4076 & 129 & numerical trouble & 8522625.081 \\
288\_22\_8 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar. homog. & 8315 & 207 & opt & 6934161.75 \\
288\_22\_8 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 3499 & 136 & numerical trouble & 8532597.119 \\
288\_22\_8 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar. homog. & 5225 & 165 & opt & 6934161.773 \\
672\_22\_8\_cli & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 13406 & 167 & numerical trouble & 7181820.191 \\
672\_22\_8\_cli & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar. homog. & 26256 & 283 & opt & 6644934.557 \\
672\_22\_8\_cli & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 11661 & 198 & numerical trouble & 7244428.474 \\
672\_22\_8\_cli & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar. homog. & 19352 & 244 & opt & 6644934.579 \\
Adalpert & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 38645 & 386 & opt & 72477.23874 \\
Adalpert & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 21013 & 328 & subopt & 72573.57534 \\
BEAM\_4032\_11\_8\_CLI & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 66684 & 232 & numerical trouble & 4185193440 \\
BEAM\_4032\_11\_8\_CLI & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 35987 & 164 & numerical trouble & 5853866007 \\
CHL\_MYR & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 4874 & 194 & opt & 2.235593851e+10 \\
CHL\_MYR & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 4293 & 239 & opt & 2.235594144e+10 \\
CN\_2025\_1 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 747 & 42 & opt & -690141646.4 \\
CN\_2025\_1 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 677 & 46 & opt & -690141585.7 \\
CN\_2025\_2 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 741 & 41 & opt & -805838755.7 \\
CN\_2025\_2 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 677 & 46 & opt & -805838660.7 \\
CN\_2025\_3 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 787 & 47 & opt & -1093066275 \\
CN\_2025\_3 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 657 & 46 & opt & -1093066102 \\
CN\_2045\_1 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 1030 & 58 & opt & 974296360.9 \\
CN\_2045\_1 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 806 & 63 & opt & 974296606.1 \\
CN\_2045\_2 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 950 & 58 & opt & 121056270.4 \\
CN\_2045\_2 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 754 & 60 & opt & 121056285.3 \\
CN\_2045\_3 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 755 & 43 & opt & -526090267.2 \\
CN\_2045\_3 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 679 & 47 & opt & -526090285.4 \\
CR\_2025 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 426 & 55 & opt & -3.207358143e+10 \\
CR\_2025 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 389 & 56 & opt & -3.207358576e+10 \\
CR\_2026 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 487 & 58 & opt & -3.203472789e+10 \\
CR\_2026 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 444 & 53 & opt & -3.203472807e+10 \\
CR\_2027 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 507 & 54 & opt & -3.289266155e+10 \\
CR\_2027 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 426 & 58 & opt & -3.289267197e+10 \\
DTU\_Y3FF\_S52\_T48\_C5 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 2078 & 119 & numerical trouble & 8.824893092e+12 \\
DTU\_Y3FF\_S52\_T48\_C5 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar. homog. & 1220 & 44 & infeas & not found \\
DTU\_Y3FF\_S52\_T48\_C5 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 4321 & 275 & numerical trouble & 5.42946747e+11 \\
DTU\_Y3FF\_S52\_T48\_C5 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar. homog. & 839 & 44 & infeas & not found \\
\makecell[l]{ELMOD\_438\_20\_noVEnam \\ es} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 14 & 0 & infeas/unbounded & not found \\
\makecell[l]{ELMOD\_438\_20\_noVEnam \\ es} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 14 & 0 & infeas/unbounded & not found \\
Gunilpert & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 27808 & 468 & opt & 61043.67456 \\
Gunilpert & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 16468 & 343 & opt & 61043.70093 \\
JRC-EU-TIMES-30-12ts & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 10 & 0 & infeas/unbounded & not found \\
JRC-EU-TIMES-30-12ts & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 10 & 0 & infeas/unbounded & not found \\
\makecell[l]{JRC-EU-TIMES-dispatc \\ h-30-2016ts.mps} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 162 & 0 & infeas/unbounded & not found \\
\makecell[l]{JRC-EU-TIMES-dispatc \\ h-30-2016ts.mps} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 165 & 0 & infeas/unbounded & not found \\
\makecell[l]{SWITCH-China-open-mo \\ del-32-433ts} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 152 & 76 & subopt & 3.193473079e+12 \\
\makecell[l]{SWITCH-China-open-mo \\ del-32-433ts} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 113 & 84 & subopt & 3.193472663e+12 \\
\makecell[l]{TIMES-GEO-global-bas \\ e-31-20ts} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 818 & 174 & opt & 241237941 \\
\makecell[l]{TIMES-GEO-global-bas \\ e-31-20ts} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 770 & 174 & opt & 241238059.9 \\
\makecell[l]{TIMES-GEO-global-net \\ zero-31-20ts} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 1132 & 260 & opt & 217369405.6 \\
\makecell[l]{TIMES-GEO-global-net \\ zero-31-20ts} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 922 & 253 & opt & 217369449.8 \\
TIMES-STEM-15-1h & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 19 & 0 & infeas/unbounded & not found \\
TIMES-STEM-15-1h & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 20 & 0 & infeas/unbounded & not found \\
\makecell[l]{YSSP\_disp\_488r\_t\_146 \\ 0b\_novenames} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 6102 & 120 & opt & 26760758.75 \\
\makecell[l]{YSSP\_disp\_488r\_t\_146 \\ 0b\_novenames} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 4606 & 122 & opt & 26760753.13 \\
\makecell[l]{ethos\_fine\_europe\_60 \\ tp-175-720ts} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 28861 & 380 & numerical trouble & 1530885597 \\
\makecell[l]{ethos\_fine\_europe\_60 \\ tp-175-720ts} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar. homog. & 8808 & 106 & numerical trouble & 3047.413832 \\
\makecell[l]{ethos\_fine\_europe\_60 \\ tp-175-720ts} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 8802 & 198 & numerical trouble & 1368089125 \\
\makecell[l]{ethos\_fine\_europe\_60 \\ tp-175-720ts} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar. homog. & 5495 & 108 & numerical trouble & 2867.039189 \\
fxe6qfja & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 20885 & 30 & numerical trouble & -1.83588975e+16 \\
fxe6qfja & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 12463 & 30 & numerical trouble & -1.833389797e+16 \\
\makecell[l]{genx-elec\_co2-15-168 \\ h} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 5630 & 153 & opt & 316331.3874 \\
\makecell[l]{genx-elec\_co2-15-168 \\ h} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 3694 & 154 & opt & 316331.4443 \\
\makecell[l]{genx-elec\_trex-15-16 \\ 8h} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 4412 & 137 & opt & 316139.1222 \\
\makecell[l]{genx-elec\_trex-15-16 \\ 8h} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 3150 & 153 & opt & 316138.9882 \\
\makecell[l]{genx-elec\_trex\_co2-1 \\ 5-168h} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 6185 & 203 & opt & 306005.2451 \\
\makecell[l]{genx-elec\_trex\_co2-1 \\ 5-168h} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 4046 & 184 & opt & 306005.8769 \\
nagsys\_subCWE\_3h & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 11107 & 418 & opt & 3919928.802 \\
nagsys\_subCWE\_3h & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 11823 & 448 & opt & 3919926.304 \\
nagsys\_subEU\_8h & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 18231 & 356 & opt & 8027060.703 \\
nagsys\_subEU\_8h & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 15354 & 349 & opt & 8027050.106 \\
nagsys\_subFR\_1h & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 6337 & 434 & opt & 854141.7328 \\
nagsys\_subFR\_1h & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 6253 & 440 & opt & 854141.6197 \\
\makecell[l]{nt2030\_2030\_CY2009\_s \\ t1\_120b} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 469 & 91 & opt & 643529.7996 \\
\makecell[l]{nt2030\_2030\_CY2009\_s \\ t1\_120b} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 511 & 91 & opt & 643529.8275 \\
oemofB3\_int\_125 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 41143 & 275 & opt & 1.235360932e+12 \\
oemofB3\_int\_125 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 51826 & 278 & opt & 1.23536008e+12 \\
oemofB3\_int\_250 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 70805 & 209 & opt & 2.627896599e+12 \\
oemofB3\_int\_250 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 72423 & 230 & opt & 2.627897104e+12 \\
oemofB3\_int\_37 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 5425 & 183 & opt & 4.411059855e+11 \\
oemofB3\_int\_37 & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 6488 & 187 & opt & 4.411059758e+11 \\
\makecell[l]{solve\_network\_myopic \\ -2030} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 86439 & 74-75 & time limit & 3.987170942e+12 \\
\makecell[l]{solve\_network\_myopic \\ -2030} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 86441 & 117-119 & time limit & 4.139290546e+12 \\
\makecell[l]{spineopt-multiyear-i \\ nvest-eu-case-study} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 6093 & 125 & opt & 1.556381858e+13 \\
\makecell[l]{spineopt-multiyear-i \\ nvest-eu-case-study} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 4553 & 133 & opt & 1.556381674e+13 \\
\makecell[l]{subCWE\_1h\_ticapin\_40 \\ b} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 41136 & 426 & subopt & 3984149.982 \\
\makecell[l]{subCWE\_1h\_ticapin\_40 \\ b} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 53955 & 583 & opt & 3910383.361 \\
\makecell[l]{zen-garden-eur-PI-an \\ nual-emission-limit-28-100ts} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 10619 & 198 & opt & 6105545.999 \\
\makecell[l]{zen-garden-eur-PI-an \\ nual-emission-limit-28-100ts} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 7367 & 203 & opt & 6105538.35 \\
\makecell[l]{zen-garden-eur-PI-co \\ nstrained-expansion-28-100ts} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 16 & bar & 15711 & 298 & opt & 6162380.261 \\
\makecell[l]{zen-garden-eur-PI-co \\ nstrained-expansion-28-100ts} & \makecell[l]{Gurobi  \\ v13.0.0rc1} & 32 & bar & 10868 & 310 & opt & 6162383.244 \\
\hline
\caption{Overview Experiments Shared Memory IPM. \\
Hardware: Intel(R) Xeon(R) Gold 6342 CPU @ 2.80GHz. \\
Barrier Convergence Tolerance: 1e-6}
\end{longtable}


\begin{longtable}{llllllll}
\hline
Instance & Solver & Thr & Method & Time & Iter & Status & Obj \\
\hline
\endfirsthead
\hline
Instance & Solver & Thr & Method & Time & Iter & Status & Obj \\
\hline
\endhead
288\_22\_8 & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 5808 & 114 & opt & 6934224.871 \\
288\_22\_8 & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 6448 & 109 & opt & 6934219.805 \\
672\_22\_8\_cli & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 59529 & 270 & numerical trouble & 6689614.248 \\
672\_22\_8\_cli & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 82259 & 219-291 & \makecell[l]{numerical trouble, \\ unfinished} & 6766892.203 \\
Adalpert & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 52952 & 231 & opt & 72476.94206 \\
Adalpert & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 51276 & 212 & opt & 72476.96883 \\
DTU\_Y3FF\_S52\_T48\_C5 & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 592 & 17 & infeas & 1.435497281e+15 \\
DTU\_Y3FF\_S52\_T48\_C5 & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 669 & 17 & infeas & 1.435497281e+15 \\
\makecell[l]{ELMOD\_438\_20\_noVEnam \\ es} & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 20 & 0 & infeas & 0 \\
\makecell[l]{ELMOD\_438\_20\_noVEnam \\ es} & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 20 & 0 & infeas & 0 \\
JRC-EU-TIMES-30-12ts & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 9 & 0 & infeas & 0 \\
JRC-EU-TIMES-30-12ts & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 9 & 0 & infeas & 0 \\
\makecell[l]{JRC-EU-TIMES-dispatc \\ h-30-2016ts} & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 587 & 64 & opt & 1033142.947 \\
\makecell[l]{JRC-EU-TIMES-dispatc \\ h-30-2016ts} & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 877 & 119 & opt & 1033331.158 \\
\makecell[l]{SWITCH-China-open-mo \\ del-32-433ts} & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 175 & 64 & opt & 3.193475215e+12 \\
\makecell[l]{SWITCH-China-open-mo \\ del-32-433ts} & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 194 & 63 & opt & 3.193473477e+12 \\
\makecell[l]{TIMES-GEO-global-bas \\ e-31-20ts} & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 4625 & 182 & opt & 241238185.1 \\
\makecell[l]{TIMES-GEO-global-bas \\ e-31-20ts} & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 4759 & 177 & opt & 241238454.4 \\
\makecell[l]{TIMES-GEO-global-net \\ zero-31-20ts} & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 2841 & 270 & opt & 217369675.3 \\
\makecell[l]{TIMES-GEO-global-net \\ zero-31-20ts} & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 20634 & 500 & unfinished & 231770194.2 \\
TIMES-STEM-15-1h & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 21 & 0 & infeas & 0 \\
TIMES-STEM-15-1h & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 24 & 0 & infeas & 0 \\
\makecell[l]{YSSP\_disp\_488r\_t\_146 \\ 0b\_novenames} & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 9720 & 72 & opt & 26760746.44 \\
\makecell[l]{YSSP\_disp\_488r\_t\_146 \\ 0b\_novenames} & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 5214 & 68 & opt & 26760754.57 \\
\makecell[l]{elec\_s\_DE5\_AT10\_lv1. \\ 0\_\_Co2L0p79-120h-T-H-B-I-W\_2015} & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 21927 & 59 & numerical trouble & 2.261682792e+15 \\
\makecell[l]{elec\_s\_DE5\_AT10\_lv1. \\ 0\_\_Co2L0p79-120h-T-H-B-I-W\_2015} & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 50198 & 59 & numerical trouble & 1.48075918e+15 \\
\makecell[l]{ethos\_fine\_europe\_60 \\ tp-175-720ts} & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 21655 & 109 & opt & 321.5173237 \\
\makecell[l]{ethos\_fine\_europe\_60 \\ tp-175-720ts} & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 16644 & 115 & opt & 321.5176666 \\
fxe6qfja & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 19988 & 141 & opt & 1197937723 \\
fxe6qfja & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 44728 & 154 & opt & 1197936725 \\
\makecell[l]{genx-elec\_co2-15-168 \\ h} & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 1532 & 184 & opt & 316331.5278 \\
\makecell[l]{genx-elec\_co2-15-168 \\ h} & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 1803 & 173 & opt & 316331.4846 \\
\makecell[l]{genx-elec\_trex-15-16 \\ 8h} & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 1442 & 167 & opt & 316139.1684 \\
\makecell[l]{genx-elec\_trex-15-16 \\ 8h} & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 1861 & 166 & opt & 316139.1524 \\
\makecell[l]{genx-elec\_trex\_co2-1 \\ 5-168h} & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 1528 & 177 & opt & 306006.7886 \\
\makecell[l]{genx-elec\_trex\_co2-1 \\ 5-168h} & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 1903 & 175 & opt & 306005.8542 \\
\makecell[l]{nt2030\_2030\_CY2009\_s \\ t1\_120b} & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 705 & 69 & opt & 643530.3271 \\
\makecell[l]{nt2030\_2030\_CY2009\_s \\ t1\_120b} & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 752 & 63 & opt & 643531.9468 \\
oemofB3\_int\_125 & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 29729 & 0 & unfinished & 8.42419127e+19 \\
oemofB3\_int\_125 & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 31183 & 0 & unfinished & 8.42419127e+19 \\
oemofB3\_int\_250 & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 117678 & 0 & unfinished & 0 \\
oemofB3\_int\_250 & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 116314 & 0 & unfinished & 0 \\
\makecell[l]{solve\_network\_myopic \\ -2030} & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 7965 & 150 & opt & 1.942316997e+12 \\
\makecell[l]{solve\_network\_myopic \\ -2030} & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 9397 & 153 & opt & 1.942321049e+12 \\
\makecell[l]{spineopt-multiyear-i \\ nvest-eu-case-study} & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 5159 & 85 & opt & 1.556382204e+13 \\
\makecell[l]{spineopt-multiyear-i \\ nvest-eu-case-study} & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 3968 & 86 & opt & 1.556382419e+13 \\
\makecell[l]{zen-garden-eur-PI-an \\ nual-emission-limit-28-100ts} & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 7932 & 117 & opt & 6105544.411 \\
\makecell[l]{zen-garden-eur-PI-an \\ nual-emission-limit-28-100ts} & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 6623 & 106 & opt & 6105561.504 \\
\makecell[l]{zen-garden-eur-PI-co \\ nstrained-expansion-28-100ts} & \makecell[l]{Xpress  \\ v9.8.0} & 16 & bar & 10023 & 179 & opt & 6162411.739 \\
\makecell[l]{zen-garden-eur-PI-co \\ nstrained-expansion-28-100ts} & \makecell[l]{Xpress  \\ v9.8.0} & 32 & bar & 7540 & 173 & opt & 6162414.698 \\
\hline
\caption{Overview Experiments Shared Memory IPM. \\
Hardware: Intel(R) Xeon(R) Gold 6342 CPU @ 2.80GHz. \\
Barrier Convergence Tolerance: 1e-6 for rel. duality gap}
\end{longtable}

\begin{longtable}{llllllll}
\hline
Instance & Solver & Thr & Method & Time & Iter & Status & Obj \\
\hline
\endfirsthead
\hline
Instance & Solver & Thr & Method & Time & Iter & Status & Obj \\
\hline
\endhead
288\_22\_8 & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 371.565 & 197400 & Optimal & 6.93416174e+06 \\
672\_22\_8\_cli & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 301.572 & 61000 & Optimal & 6.64461210e+06 \\
Adalpert & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 1808.148 & 209000 & Optimal & 7.24794209e+04 \\
BEAM\_2016\_11\_8 & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 1397.361 & 182600 & Optimal & 6.96050711e+06 \\
BEAM\_4032\_11\_8\_CLI & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & inf &  \\
CHL\_MYR & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & \makecell[l]{inf PSLP \\
presolve} &  \\
CN\_2025\_1 & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & \makecell[l]{inf PSLP \\
presolve} &  \\
CN\_2025\_2 & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & \makecell[l]{inf PSLP \\
presolve} &  \\
CN\_2025\_3 & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & \makecell[l]{inf PSLP \\
presolve} &  \\
CN\_2045\_1 & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & \makecell[l]{inf PSLP \\
presolve} &  \\
CN\_2045\_2 & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & \makecell[l]{inf PSLP \\
presolve} &  \\
CN\_2045\_3 & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & \makecell[l]{inf PSLP \\
presolve} &  \\
CR\_2025 & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & \makecell[l]{inf PSLP \\
presolve} &  \\
CR\_2026 & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & \makecell[l]{inf PSLP \\
presolve} &  \\
CR\_2027 & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & \makecell[l]{inf PSLP \\
presolve} &  \\
DTU\_Y3FF\_S52\_T48\_C5 & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & \makecell[l]{CUDA \\
issue} &  \\
\makecell[l]{elec\_s\_DE5\_AT10\_lv1.0\_\_Co \\
2L0p79-120h-T-H-B-I-W\_2015} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & to run &  \\
\makecell[l]{ELMOD\_438\_2 \\
0\_noVEnames} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & inf &  \\
\makecell[l]{ELMOD\_876\_1 \\
0\_noVEnames} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & \makecell[l]{crash in PSLP \\
presolve} &  \\
\makecell[l]{ethos\_fine\_europ \\
e\_60tp-175-720ts} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 16574.279 & 21496400 & Optimal & 3.21604010e+02 \\
full\_1h\_ticapin\_120b & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & \makecell[l]{crash in PSLP \\
presolve} &  \\
fxe6qfja & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 7058.344 & 3822600 & Optimal & 1.19837308e+09 \\
\makecell[l]{genx-elec\_ \\
co2-15-168h} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 1620.571 & 1617400 & Optimal & 3.16333731e+05 \\
\makecell[l]{genx-elec\_t \\
rex-15-168h} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 643.509 & 920400 & Optimal & 3.16141997e+05 \\
\makecell[l]{genx-elec\_tre \\
x\_co2-15-168h} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 1044.336 & 747200 & Optimal & 3.06005231e+05 \\
Gunilpert & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 720.359 & 244600 & Optimal & 6.10508626e+04 \\
JRC-EU-TIMES-30-12ts & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & inf &  \\
\makecell[l]{JRC-EU-TIMES-di \\
spatch-30-2016ts} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & \makecell[l]{inf PSLP \\
presolve} &  \\
nagsys\_subCWE\_3h & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 3093.957 & 1082400 & Optimal & 3.95604071e+06 \\
nagsys\_subEU\_8h & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 2227.701 & 744600 & Optimal & 8.23924929e+06 \\
nagsys\_subFR\_1h & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 3097.397 & 1563600 & Optimal & 8.65672429e+05 \\
\makecell[l]{nt2030\_2030\_C \\
Y2009\_st1\_120b} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 644.025 & 577600 & Optimal & 6.43529880e+05 \\
oemofB3\_int\_125 & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & to run &  \\
oemofB3\_int\_250 & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & to run &  \\
oemofB3\_int\_37 & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & to run &  \\
OTAI\_b-ts5\_cplex & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 4841.422 & 1432600 & Optimal & 4.89327325e+04 \\
phoenix2 & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 237.570 & 123800 & Optimal & -6.35226692e+11 \\
pypsa-de-elec-50-1h & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 178.155 & 194200 & Optimal & -5.64704766e+09 \\
pypsa-de-sec-20-1h & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 8347.517 & 3195600 & Optimal & 7.14017675e+10 \\
\makecell[l]{pypsa-eur- \\
elec-100-3h} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 189.221 & 267400 & Optimal & 3.49635267e+10 \\
\makecell[l]{solve\_networ \\
k\_myopic-2030} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 3755.122 & 2162600 & Optimal & 1.93125856e+12 \\
\makecell[l]{spineopt-multiyear- \\
invest-eu-case-study} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & \makecell[l]{inf PSLP \\
presolve} &  \\
\makecell[l]{subCWE\_1h\_ \\
ticapin\_40b} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 27939.512 & 3139200 & Optimal & 3.94585399e+06 \\
\makecell[l]{SWITCH-China-ope \\
n-model-32-433ts} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 148.011 & 236400 & Optimal & 3.44720450e+12 \\
\makecell[l]{TIMES-GEO-glob \\
al-base-31-20ts} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 100.307 & 154200 & Optimal & 2.41101412e+08 \\
\makecell[l]{TIMES-GEO-global \\
-netzero-31-20ts} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 198.602 & 376400 & Optimal & 2.15668524e+08 \\
TIMES-STEM-15-1h & \makecell{cuOPT \\ (version ?)} & 26 & PDLP &  &  & inf &  \\
\makecell[l]{YSSP\_disp\_488r\_t \\
\_1460b\_novenames} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 65164.175 & 19029000 & Optimal & 2.65986012e+07 \\
\makecell[l]{zen-garden-eur-PI-annual \\
-emission-limit-28-100ts} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 86400.085 & 123853400 & Time Limit & 6.10557568e+06 \\
\makecell[l]{zen-garden-eur-PI-constr \\
ained-expansion-28-100ts} & \makecell{cuOPT \\ (version ?)} & 26 & PDLP & 41074.246 & 58258400 & Optimal & 6.16239985e+06 \\
\hline
\caption{Overview Experiments cuOPT. \\
Hardware: H100 ("gpu910" and "gpu911") \\
Convergence Tolerance: 1e-6 for both rel. primal and rel. dual tolerance}
\end{longtable}

\begin{longtable}{llllllll}
\hline
Instance & Solver & Thr & Method & Time & Iter & Status & Obj \\
\hline
\endfirsthead
\hline
Instance & Solver & Thr & Method & Time & Iter & Status & Obj \\
\hline
\endhead
288\_22\_8 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 2754.71 & 116 & ? & 6.9341617227e+06 \\
288\_22\_8 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 3327.01 & 116 & ? & 6.9341617731e+06 \\
672\_22\_8\_cli & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 16918.36 & 178 & ? & 6.6449343553e+06 \\
672\_22\_8\_cli & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 15321.55 & 177 & ? & 6.6449343401e+06 \\
Adalpert & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 42510.21 & 234 & ? & 7.2476838276e+04 \\
Adalpert & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 34669.70 & 228 & ? & 7.2476838305e+04 \\
BEAM\_2016\_11\_8 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 26948.96 & 204 & ? & 6.9604891703e+06 \\
BEAM\_2016\_11\_8 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 22887.70 & 192 & ? & 6.9604892295e+06 \\
BEAM\_4032\_11\_8\_CLI & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} &  &  & to run &  \\
BEAM\_4032\_11\_8\_CLI & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} &  &  & to run &  \\
CHL\_MYR & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 2352.44 & 135 & ? & 2.2355926487e+10 \\
CHL\_MYR & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 2243.81 & 139 & ? & 2.2355926486e+10 \\
CN\_2025\_1 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 945.14 & 38 & ? & -6.9014204097e+08 \\
CN\_2025\_1 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 832.83 & 38 & ? & -6.9014204075e+08 \\
CN\_2025\_2 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 764.48 & 41 & ? & -8.0583905884e+08 \\
CN\_2025\_2 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 718.45 & 41 & ? & -8.0583906006e+08 \\
CN\_2025\_3 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 1039.27 & 40 & ? & -1.0930663890e+09 \\
CN\_2025\_3 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 971.38 & 40 & ? & -1.0930663899e+09 \\
CN\_2045\_1 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 1095.63 & 49 & ? & 9.7429631989e+08 \\
CN\_2045\_1 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 940.28 & 49 & ? & 9.7429631983e+08 \\
CN\_2045\_2 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 913.60 & 42 & ? & 1.2105628432e+08 \\
CN\_2045\_2 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 783.24 & 43 & ? & 1.2105626495e+08 \\
CN\_2045\_3 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 642.72 & 37 & ? & -5.2609028724e+08 \\
CN\_2045\_3 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 605.81 & 37 & ? & -5.2609028724e+08 \\
CR\_2025 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 489.46 & 40 & ? & -3.2073591802e+10 \\
CR\_2025 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 542.38 & 44 & ? & -3.2073594795e+10 \\
CR\_2026 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 528.70 & 42 & ? & -3.2034740184e+10 \\
CR\_2026 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 475.92 & 38 & ? & -3.2034732547e+10 \\
CR\_2027 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 519.55 & 44 & ? & -3.2892680508e+10 \\
CR\_2027 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 545.12 & 45 & ? & -3.2892680386e+10 \\
DTU\_Y3FF\_S52\_T48\_C5 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} &  &  & inf &  \\
DTU\_Y3FF\_S52\_T48\_C5 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} &  &  & inf &  \\
\makecell[l]{elec\_s\_DE5\_AT10\_lv1.0\_\_Co \\
2L0p79-120h-T-H-B-I-W\_2015} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} &  &  & inf &  \\
\makecell[l]{elec\_s\_DE5\_AT10\_lv1.0\_\_Co \\
2L0p79-120h-T-H-B-I-W\_2015} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} &  &  & inf &  \\
\makecell[l]{ELMOD\_438\_2 \\
0\_noVEnames} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} &  &  & inf &  \\
\makecell[l]{ELMOD\_438\_2 \\
0\_noVEnames} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} &  &  & inf &  \\
\makecell[l]{ELMOD\_876\_1 \\
0\_noVEnames} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 19253.28 & 100 & ? & 7.9065871689e+04 \\
\makecell[l]{ELMOD\_876\_1 \\
0\_noVEnames} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 18657.28 & 101 & ? & 7.9065899879e+04 \\
\makecell[l]{ethos\_fine\_europ \\
e\_60tp-175-720ts} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 10278.29 & 107 & ? & 3.3110554738e+02 \\
\makecell[l]{ethos\_fine\_europ \\
e\_60tp-175-720ts} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 7768.57 & 106 & ? & 3.3103363892e+02 \\
\makecell[l]{full\_1h\_t \\
icapin\_120b} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} &  &  & mem &  \\
\makecell[l]{full\_1h\_t \\
icapin\_120b} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} &  &  & mem &  \\
fxe6qfja & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 3988.64 & 118 & ? & 1.1979776513e+09 \\
fxe6qfja & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 3440.18 & 126 & ? & 1.1979845055e+09 \\
\makecell[l]{genx-elec\_ \\
co2-15-168h} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 869.10 & 117 & ? & 3.1633215781e+05 \\
\makecell[l]{genx-elec\_ \\
co2-15-168h} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 930.95 & 121 & ? & 3.1633139814e+05 \\
\makecell[l]{genx-elec\_t \\
rex-15-168h} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 1446.82 & 156 & ? & 3.1613882794e+05 \\
\makecell[l]{genx-elec\_t \\
rex-15-168h} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 1520.80 & 154 & ? & 3.1613882834e+05 \\
\makecell[l]{genx-elec\_tre \\
x\_co2-15-168h} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 1177.26 & 163 & ? & 3.0600631061e+05 \\
\makecell[l]{genx-elec\_tre \\
x\_co2-15-168h} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 1138.83 & 145 & ? & 3.0600631393e+05 \\
Gunilpert & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 11371.12 & 227 & ? & 6.1043386693e+04 \\
Gunilpert & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 9399.39 & 244 & ? & 6.1043364123e+04 \\
JRC-EU-TIMES-30-12ts & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} &  &  & inf &  \\
JRC-EU-TIMES-30-12ts & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} &  &  & inf &  \\
\makecell[l]{JRC-EU-TIMES-di \\
spatch-30-2016ts} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 2227.89 & 131 & ? & 1.0330382560e+06 \\
\makecell[l]{JRC-EU-TIMES-di \\
spatch-30-2016ts} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 2030.50 & 140 & ? & 1.0330381653e+06 \\
nagsys\_subCWE\_3h & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 8002.97 & 270 & ? & 3.9198933533e+06 \\
nagsys\_subCWE\_3h & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 7274.29 & 278 & ? & 3.9198945639e+06 \\
nagsys\_subEU\_8h & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & Limit reached  & 1360 & ? & 8.0275304949e+06 \\
nagsys\_subEU\_8h & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 77623.66 & 1352 & ? & 8.0271771344e+06 \\
nagsys\_subFR\_1h & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 4741.67 & 309 & ? & 8.5413174144e+05 \\
nagsys\_subFR\_1h & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 4483.99 & 310 & ? & 8.5413174058e+05 \\
\makecell[l]{nt2030\_2030\_C \\
Y2009\_st1\_120b} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 640.95 & 76 & ? & 6.4352975148e+05 \\
\makecell[l]{nt2030\_2030\_C \\
Y2009\_st1\_120b} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 585.02 & 76 & ? & 6.4352975148e+05 \\
oemofB3\_int\_125 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 14738.32 & 310 & ? & 1.2354278609e+12 \\
oemofB3\_int\_125 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 21801.93 & 348 & ? & 1.2354425024e+12 \\
oemofB3\_int\_250 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} &  &  & to run &  \\
oemofB3\_int\_250 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} &  & & mem &  \\
oemofB3\_int\_37 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 3744.32 & 240 & ? & 4.4113246169e+11 \\
oemofB3\_int\_37 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 3568.56 & 227 & ? & 4.4113642581e+11 \\
OTAI\_b-ts5\_cplex & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 6027.86 & 198 & ? & 4.8920435355e+04 \\
OTAI\_b-ts5\_cplex & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 5988 & 203 & ? & 89 \\
phoenix2 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 2028.45 & 140 & ? & -6.3523254491e+11 \\
phoenix2 & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 2118.05 & 145 & ? & -6.3523252098e+11 \\
pypsa-de-elec-50-1h & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 2244.60 & 109 & ? & 5.6493695262e+09 \\
pypsa-de-elec-50-1h & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 1946.53 & 109 & ? & 5.6493697743e+09 \\
pypsa-de-sec-20-1h & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 3714.26 & 131 & ? & 8.1420995411e+10 \\
pypsa-de-sec-20-1h & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 3415.37 & 134 & ? & 8.1420906917e+10 \\
\makecell[l]{pypsa-eur- \\
elec-100-3h} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 784.39 & 63 & ? & 3.4963390459e+10 \\
\makecell[l]{pypsa-eur- \\
elec-100-3h} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 722.92 & 63 & ? & 3.4963390479e+10 \\
\makecell[l]{solve\_networ \\
k\_myopic-2030} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 4451.33 & 145 & ? & 1.9423111294e+12 \\
\makecell[l]{solve\_networ \\
k\_myopic-2030} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 3671.06 & 145 & ? & 1.9423111083e+12 \\
\makecell[l]{spineopt-multiyear- \\
invest-eu-case-study} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 11824.24 & 431 & ? & 1.5563391059e+13 \\
\makecell[l]{spineopt-multiyear- \\
invest-eu-case-study} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 2351.86 & 90 & ? & 1.5563833495e+13 \\
\makecell[l]{subCWE\_1h\_ \\
ticapin\_40b} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 29989.74 & 284 & ? & 3.9103521370e+06 \\
\makecell[l]{subCWE\_1h\_ \\
ticapin\_40b} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 27452.99 & 279 & ? & 3.9103524571e+06 \\
\makecell[l]{SWITCH-China-ope \\
n-model-32-433ts} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 343.42 & 70 & ? & 3.1934717403e+12 \\
\makecell[l]{SWITCH-China-ope \\
n-model-32-433ts} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 333.32 & 70 & ? & 3.1934717437e+12 \\
\makecell[l]{TIMES-GEO-glob \\
al-base-31-20ts} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 1324.60 & 134 & ? & 2.4123788406e+08 \\
\makecell[l]{TIMES-GEO-glob \\
al-base-31-20ts} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 1113.29 & 134 & ? & 2.4123788406e+08 \\
\makecell[l]{TIMES-GEO-global \\
-netzero-31-20ts} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 967.61 & 139 & ? & 2.1736857591e+08 \\
\makecell[l]{TIMES-GEO-global \\
-netzero-31-20ts} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 878.71 & 139 & ? & 2.1736857591e+08 \\
TIMES-STEM-15-1h & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} &  &  & inf &  \\
TIMES-STEM-15-1h & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} &  &  & inf &  \\
\makecell[l]{YSSP\_disp\_4 \\
88r\_t\_1460b} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} &  &  & mem &  \\
\makecell[l]{YSSP\_disp\_4 \\
88r\_t\_1460b} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} &  &  & mem &  \\
\makecell[l]{zen-garden-eur-PI-annual \\
-emission-limit-28-100ts} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 8787.43 & 147 & ? & 6.1057037588e+06 \\
\makecell[l]{zen-garden-eur-PI-annual \\
-emission-limit-28-100ts} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 6385.52 & 147 & ? & 6.1057332945e+06 \\
\makecell[l]{zen-garden-eur-PI-constr \\
ained-expansion-28-100ts} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 16 & \makecell{int.-point \\ optimizer} & 12545.65 & 212 & ? & 6.1661389494e+06 \\
\makecell[l]{zen-garden-eur-PI-constr \\
ained-expansion-28-100ts} & \makecell{MOSEK 11.1.5 \\ (from GAMS 53.1.0)} & 32 & \makecell{int.-point \\ optimizer} & 8968.75 & 207 & ? & 6.1647124558e+06 \\
\hline
\caption{Overview Experiments MOSEK. \\
Hardware: Intel(R) Xeon(R) Gold 6342 CPU @ 2.80GHz. \\
Convergence Tolerance: 1e-6 for relative gap and for both primal and dual feasibility}
\end{longtable}

